N$^2$M$^2$: Learning Navigation for Arbitrary Mobile Manipulation Motions in Unseen and Dynamic Environments

Despite its importance in both industrial and service robotics, mobile manipulation remains a significant challenge as it requires a seamless integration of end-effector trajectory generation with navigation skills as well as reasoning over long-horizons. Existing methods struggle to control the large configuration space, and to navigate dynamic and unknown environments. In previous work, we proposed to decompose mobile manipulation tasks into a simplified motion generator for the end-effector in task space and a trained reinforcement learning agent for the mobile base to account for kinematic feasibility of the motion. In this work, we introduce Neural Navigation for Mobile Manipulation (N$^2$M$^2$) which extends this decomposition to complex obstacle environments and enables it to tackle a broad range of tasks in real world settings. The resulting approach can perform unseen, long-horizon tasks in unexplored environments while instantly reacting to dynamic obstacles and environmental changes. At the same time, it provides a simple way to define new mobile manipulation tasks. We demonstrate the capabilities of our proposed approach in extensive simulation and real-world experiments on multiple kinematically diverse mobile manipulators. Code and videos are publicly available at http://mobile-rl.cs.uni-freiburg.de.

==> images/tex_figures/astar_weights.tex <==
\begin{figure}
    \footnotesize
	\centering
  		\includegraphics[width=1.0\columnwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip,angle =0]{images/envs/astar_weights.png}
  		\vspace{-0.5cm}
	\caption{Astar weights}
  	\label{fig:astar_weights}
\end{figure}

==> images/tex_figures/non_convex.tex <==
\setlength{\tabcolsep}{0pt}
\renewcommand{\arraystretch}{1}
\begin{figure*}
	\centering
	\resizebox{1\textwidth}{!}{%
	\begin{tabular}{cccc}
	    \includegraphics[width=1\textwidth,trim={7.0cm 0.0cm 7.0cm 0.0cm},clip,angle=0]{images/non_convex/0.png} &
	    \includegraphics[width=1\textwidth,trim={7.0cm 0.0cm 7.0cm 0.0cm},clip,angle=0]{images/non_convex/1.png} &
	    \includegraphics[width=1\textwidth,trim={7.0cm 0.0cm 7.0cm 0.0cm},clip,angle=0]{images/non_convex/2.png} &
        \includegraphics[width=1\textwidth,trim={7.0cm 0.0cm 7.0cm 0.0cm},clip,angle=0]{images/non_convex/5.png}\\
	    \end{tabular}
        }
	\caption{Examples of the agents navigating non-convex obstacles in the analytical environment. Non-convex obstacles in the proximity of the agent are marked in red.}
  	\label{fig:nonconvex}
\end{figure*}
\setlength{\tabcolsep}{6pt}
\renewcommand{\arraystretch}{1}

==> images/tex_figures/non_convex2.tex <==
\setlength{\tabcolsep}{1pt}
\renewcommand{\arraystretch}{1}
\begin{figure*}
	\centering
	\resizebox{1\textwidth}{!}{%
	\begin{tabular}{ccc}
	    % \includegraphics[width=0.33\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip,angle=0]{images/non_convex/0.png} &
	    % \includegraphics[width=0.33\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip,angle=0]{images/non_convex/1.png} &
	    % \includegraphics[width=0.33\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip,angle=0]{images/non_convex/2.png}\\
     \includegraphics[width=0.3\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip,angle=0]{images/non_convex/pr2_corner.png} &
     \includegraphics[width=0.48\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip,angle=0]{images/non_convex/pr2_door.png} &
     \includegraphics[width=0.217\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip,angle=0]{images/non_convex/hsr_door.png} \\
	    \end{tabular}
        }
	\caption{Examples of the agents navigating non-convex obstacles in the real world. Left: the PR2 navigates around non-convex corners and edges of the environment. Middle and right: the door forms a non-convex obstacle with the door frame while opening it and driving through it.}
  	\label{fig:nonconvex2}
\end{figure*}
\setlength{\tabcolsep}{6pt}
\renewcommand{\arraystretch}{1}

==> tables/fmm_comparison.tex <==
\begin{table*}
    \centering
    \caption{Success rates for experiments in the analytical environment.} 
    \begin{threeparttable}
    \begin{tabularx}{\textwidth}{cl|YYYYY|YYY|Y|Y}
    \toprule
           & & \multicolumn{5}{c|}{$A^*$-slerp} & \multicolumn{3}{c|}{Imitation Learning} & \multicolumn{1}{c|}{Spline} & \multicolumn{1}{c}{Avg} \\ %& \multicolumn{2}{c}{$A^*$-fwd}\\
    \cmidrule{3-12}
      & Agent                & rnd obstacle & p\&p & bookstore p\&p &  dynamic obstacle & dynamic p\&p & cabinet & drawer & door & spline & \\ %& p\&p & bookstore p\&p\\
    \midrule
        \parbox[t]{1mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{PR2}}}
        % & MPC              &   10.0       & 64.0 &                & 36.0 &      & 54.0 &   ~0.0 &     50.0 &      &            &        & \\
        & MPC                &   54.0       & 70.0 &           ~8.0 & 64.0 & 54.0 & 62.0 &   76.0 &     32.0 & 96.0 & 57.3          \\ %& 16.0 &   52.0\\
        & E2E                &   ~0.0       & ~0.0 &           ~0.0 & ~0.0 & ~0.0 & ~0.0 &   ~0.0 &     ~0.0 & ~0.0 & ~0.0          \\ %& ~0.0 &   ~0.0\\
        %&\textbf{Ours old}  &   84.8       & 97.6 &           72.0 & 86.0 &      & 97.2 &   97.6 &     98.4 & 80.4 & \textbf{85.9} \\ %& 94.4 &   62.8\\
        & \textbf{\ours}      &   86.0       & 97.6 &           70.0 & 84.4 & 81.6 & 97.2 &   97.6 &     98.4 & 80.8 & \textbf{88.2} \\ %& 94.0 &   62.0\\
        % & Ours p0.02         &   84.8       & 96.0 &           70.4 & 78.8 &      & 96.0 &   98.8 &     95.2 & 77.2 & 85.4        \\ %  & 90.4 &   66.0\\
        \cmidrule{1-12}
        \parbox[t]{1mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{HSR}}}
        %&MPC                &   28.0       & 52.0 &                &      &  & 28.0 &   ~0.0 &     ~0.0 & 80.0 &               &   \\ %     & \\
        & MPC                &   64.0       & 72.0 &           48.0 & 60.0 & 60.0 & 68.0 &   68.0 &     66.0 & 98.0 & 67.1          \\ %& 30.0 &   82.0\\
        & E2E                &   25.2       & 38.8 &           10.4 & 17.6 & 13.2 & 52.4 &   14.4 &     43.2 & 38.0 & 28.1          \\ %& 27.2 &   12.0\\
        & \textbf{\ours}      &   63.2       & 92.0 &           68.0 & 82.0 & 88.0 & 93.2 &   87.2 &     88.0 & 84.0 & \textbf{82.4} \\ %& 86.4 &   80.0\\
        \cmidrule{1-12}
        \parbox[t]{1mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{Tiago}}}
        %&MPC                &              & 38.0 &                &      &      & 25.0 &        &          &      &               \\ %&        & \\
        & MPC                &   46.0       & 68.0 &           ~0.8 & 40.0 & 30.0 & 62.0 &   52.0 &    32.0  & 86.0 & 46.3          \\ %& ~6.0 &   ~6.0\\
        %&E2E                &   ~8.0       & ~6.0 &           ~2.0 & ~4.0 &      & ~4.0 &   ~0.0 &     ~0.0 & ~0.0 &               \\ %& ~0.0 &   ~0.0\\
        & E2E                &   ~0.0       & ~0.0 &           ~0.0 & ~0.0 & ~0.0 & ~0.0 &   ~0.0 &     ~0.0 & ~0.0 & ~0.0          \\ %& ~0.0 &   ~0.0\\
        %&\textbf{Ours}      &   66.0       & 94.0 &           36.0 & 60.0 &      & 80.0 &   86.0 &     60.0 & 56.0 & \textbf{63.2} \\ %& 68.0 &   26.0\\
        %&\textbf{Ours}      &   59.6       & 88.8 &           32.8 & 52.8 &      & 83.6 &   88.4 &     57.2 & 50.0 & \textbf{61.6} \\ %& 63.6 &   38.8\\
        & \textbf{\ours}     &   61.2       & 91.6 &           42.0 & 54.4 & 50.4 & 81.6 &   89.2 &     62.4 & 56.0 & \textbf{65.4} \\ %& 68.0 &   46.0\\
        \cmidrule{1-12}
        & \multicolumn{11}{c}{trained on rndstarrndgoal -- ignoring collisions with task objects, from random initial configurations}\\
        \cmidrule{1-12}
        & Agent                & rndstarrndgoal & p\&p & p\&p top grasp, rnd height & cabinet & drawer & door & spline & Avg\\
        \cmidrule{1-12}
        \parbox[t]{1mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{Fmm}}}
        & our config & 68.0 & 42.0 & 56.0 & 42.0 & 38.0 & 38.0 & 24.0 & 44.0\\
        & 45 degree  & 86.0 & 68.0 & 72.0 & 82.0 & 66.0 & 34.0 & 48.0 & 65.1\\
        & 90 degree  & 92.0 & 82.0 & 68.0& 86.0 & 72.0 & 66.0 & 48.0 & 73.4\\
        \cmidrule{1-12}
        & \multicolumn{11}{c}{trained on rndobstacle -- with collisions and obstacles in the path (not designed for size of fmm), from random initial configurations}\\
        \cmidrule{1-12}
        & Agent                & rndstarrndgoal & p\&p & cabinet & drawer & door & rndobstacle & Avg\\
        \cmidrule{1-12}
        \parbox[t]{1mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{Fmm}}}
        & our config & 66.0 & 28.0 & 20.0 & 12.0 &  0.0 & 34.0 & 26.7\\
        & 45 degree  & 72.0 & 50.0 & 54.0 & 26.0 &  4.0 & 34.0 & 40.0\\%50.0 & 54.0 & 24.0 & 44.0 & 40.0 \\
        & 90 degree  & 74.0 & 50.0 & 50.0 & 52.0 &  8.0 & 54.0 & 48.0\\%48.0 & 54.0 & 50.0 & 12.0 & 56.0 \\
        \cmidrule{1-12}
        & \multicolumn{11}{c}{rndobstacle}\\
        & Agent                & rnd obstacle & p\&p & bookstore p\&p &  dynamic obstacle & dynamic p\&p & cabinet & drawer & door & spline & \\ %& p\&p & bookstore p\&p\\
        \cmidrule{1-12}
        \parbox[t]{1mm}{\multirow{8}{*}{\rotatebox[origin=c]{90}{Fmm}}}
        & sbl               & (60.0) 38.0 & 24.0 & &      & & 20.0 & 18.0 &  0.0 & 18.0 \\
        & ray               & (62.0) 38.0 & 18.0 & & 30.0 & & 12.0 & 20.0 &  6.0 & 12.0 \\
        & ray fs 3          & (64.0) 46.0 & 38.0 & & 48.0 & & 28.0 & 26.0 & 20.0 & 26.0 \\
        & ray fs 5          & (66.0) 40.0 & 36.0 & & 50.0 & & 28.0 & 38.0 & 30.0 & 22.0 \\
    \bottomrule
    \end{tabularx}
        \begin{tablenotes}[para,flushleft]
       \footnotesize      
       Notes: Evaluation on unseen tasks from three different motions systems, an $A^*$-based system, an imitation system learned from human demonstrations and spline interpolation of random waypoints. The last column reports the average across all tasks. We evaluate all models on three different robotic platforms, the PR2, HSR, and TIAGo.
     \end{tablenotes}
   \end{threeparttable}
    \label{tab:fmm}
\end{table*}

